Leveraging Decentralized Artificial Intelligence to Enhance Resilience of Energy Networks

This paper reintroduces the notion of resilience in the context of recent issues originated from climate change triggered events including severe hurricanes and wildfires. A recent example is PG&E's forced power outage to contain wildfire risk which led to widespread power disruption. This paper focuses on answering two questions: who is responsible for resilience? and how to quantify the monetary value of resilience? To this end, we first provide preliminary definitions of resilience for power systems. We then investigate the role of natural hazards, especially wildfire, on power system resilience. Finally, we will propose a decentralized strategy for a resilient management system using distributed storage and demand response resources. Our proposed high fidelity model provides utilities, operators, and policymakers with a clearer picture for strategic decision making and preventive decisions.

==> ref.tex <==
@misc{PG&E,
 author = { Katherine Blunt, Jim Carlton and Erin Ailworth},
 editor = {{The Wall Street Journal}},
 title = {{PG\&E Starts to Cut Power for Nearly 800,000 California Customers on Wildfire Risk}},
 url = {},
 lastchecked = {14.01.2013},
 originalyear = {18.02.2011}
}

@misc{PGE,
 author = {An S &C report in collaboration with Frost & Sullivanl},
 editor = {{}},
 title = {{S\&C’s 2018 State of Commercial \& Industrial Power Reliability Report}},
 url = {https://www.sandc.com/globalassets/sac-electric/documents/sharepoint/documents---all-documents/technical-paper-100-t120.pdf},
 lastchecked = {14.01.2013},
 originalyear = {18.02.2011}
}
@article{rogers2013noaa,
  title={NOAA'S hurricane intensity forecasting experiment: A progress report},
  author={Rogers, Robert and Aberson, Sim and Aksoy, Altug and Annane, Bachir and Black, Michael and Cione, Joseph and Dorst, Neal and Dunion, Jason and Gamache, John and Goldenberg, Stan and others},
  journal={Bulletin of the American Meteorological Society},
  volume={94},
  number={6},
  pages={859--882},
  year={2013},
  publisher={American Meteorological Society}
}

@book{rappaport1995deadliest,
  title={The deadliest Atlantic tropical cyclones, 1492-1994},
  author={Rappaport, Edward N and Fernandez-Partagas, Jose},
  year={1995},
  publisher={National Hurricane Center}
}

@misc{xxx2,
    title = "List of Florida hurricanes",
    year = "2019",
    url = "https://en.wikipedia.org/w/index.php?title=List_of_Florida_hurricanes&oldid=919377085",
    note = "[Online; accessed 6-November-2019]"
  }

@misc{Bloom,
 author = {Asim Hussain},
 editor = {{BloomEnergy}},
 title = {{A Day Without Power: Outage Costs for Businesses}},
 url = {https://www.bloomenergy.com/blog/a-day-without-power-outage-costs-businesses},
 lastchecked = {14.01.2013},
 originalyear = {18.02.2011}
}
@misc{Zillow,
 author = {Manny Garcia},
 editor = {{Zillow}},
 title = {{Almost Half a Million California Homes at Risk From Wildfires}},
 url = {https://www.zillow.com/research/california-homes-wildfire-risk-25065/},
 lastchecked = {14.01.2013},
 originalyear = {18.02.2011}
}
@misc{ wikiCal,
    author = "{Wikipedia contributors}",
    title = "2018 California wildfires --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2019",
    note = "[Online; accessed 15-October-2019]"
  }
@article{bahrami2018decentralized,
  title={A decentralized renewable generation management and demand response in power distribution networks},
  author={Bahrami, Shahab and Amini, M Hadi and Shafie-Khah, Miadreza and Catalao, Joao PS},
  journal={IEEE Transactions on Sustainable Energy},
  volume={9},
  number={4},
  pages={1783--1797},
  year={2018},
  publisher={IEEE}
}
@article{bahrami2017decentralized,
  title={A decentralized electricity market scheme enabling demand response deployment},
  author={Bahrami, Shahab and Amini, M Hadi and Shafie-khah, Miadreza and Catalao, Joao PS},
  journal={IEEE Transactions on Power Systems},
  volume={33},
  number={4},
  pages={4218--4227},
  year={2017},
  publisher={IEEE}
}

@article{gholami2018toward,
  title={Toward a consensus on the definition and taxonomy of power system resilience},
  author={Gholami, Amin and Shekari, Tohid and Amirioun, Mohammad Hassan and Aminifar, Farrokh and Amini, M Hadi and Sargolzaei, Arman},
  journal={IEEE Access},
  volume={6},
  pages={32035--32053},
  year={2018},
  publisher={IEEE}
}
@inproceedings{amini2013load,
  title={Load management using multi-agent systems in smart distribution network},
  author={Amini, Mohammad Hadi and Nabi, Behrouz and Haghifam, Mahmoud-Reza},
  booktitle={2013 IEEE Power \& Energy Society General Meeting},
  pages={1--5},
  year={2013},
  organization={IEEE}
}

@incollection{salgueiro2020multi,
  title={Multi-agent-Based Decision Support Systems in Smart Microgrids},
  author={Salgueiro, Yamisleydi and Rivera, Marco and N{\'a}poles, Gonzalo},
  booktitle={Intelligent Decision Technologies 2019},
  pages={123--132},
  year={2020},
  publisher={Springer}
}

@article{sujil2018multi,
  title={Multi agent system: concepts, platforms and applications in power systems},
  author={Sujil, A and Verma, Jatin and Kumar, Rajesh},
  journal={Artificial Intelligence Review},
  volume={49},
  number={2},
  pages={153--182},
  year={2018},
  publisher={Springer}
}

@article{liu2014decentralized,
  title={Decentralized multi-agent system-based cooperative frequency control for autonomous microgrids with communication constraints},
  author={Liu, Wei and Gu, Wei and Sheng, Wanxing and Meng, Xiaoli and Wu, Zaijun and Chen, Wu},
  journal={IEEE Transactions on Sustainable Energy},
  volume={5},
  number={2},
  pages={446--456},
  year={2014},
  publisher={IEEE}
}

@article{holling,
author = {Holling, C S},
title = {Resilience and Stability of Ecological Systems},
journal = {Annual Review of Ecology and Systematics},
volume = {4},
number = {1},
pages = {1-23},
year = {1973},
doi = {10.1146/annurev.es.04.110173.000245},

URL = { 
        https://doi.org/10.1146/annurev.es.04.110173.000245
    
},
eprint = { 
        https://doi.org/10.1146/annurev.es.04.110173.000245
    
}

}
@article{brown2006defending,
  title={Defending critical infrastructure},
  author={Brown, Gerald and Carlyle, Matthew and Salmer{\'o}n, Javier and Wood, Kevin},
  journal={Interfaces},
  volume={36},
  number={6},
  pages={530--544},
  year={2006},
  publisher={Informs}
}
@article{adger2000social,
  title={Social and ecological resilience: are they related?},
  author={Adger, W Neil},
  journal={Progress in human geography},
  volume={24},
  number={3},
  pages={347--364},
  year={2000},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}
@article{perrings2007future,
  title={Future challenges},
  author={Perrings, Charles},
  journal={Proceedings of the National Academy of Sciences},
  volume={104},
  number={39},
  pages={15179--15180},
  year={2007},
  publisher={National Acad Sciences}
}


@article{chen2019joint,
  title={A Joint Learning and Communications Framework for Federated Learning over Wireless Networks},
  author={Chen, Mingzhe and Yang, Zhaohui and Saad, Walid and Yin, Changchuan and Poor, H Vincent and Cui, Shuguang},
  journal={arXiv preprint arXiv:1909.07972},
  year={2019}
}

@incollection{amini2019sustainable,
  title={Sustainable smart cities through the lens of complex interdependent infrastructures: Panorama and state-of-the-art},
  author={Amini, M Hadi and Arasteh, Hamidreza and Siano, Pierluigi},
  booktitle={Sustainable Interdependent Networks II},
  pages={45--68},
  year={2019},
  publisher={Springer}
}

@article{amini2019distributed,
  title={Distributed Holistic Framework for Smart City Infrastructures: Tale of Interdependent Electrified Transportation Network and Power Grid},
  author={Amini, M Hadi and Mohammadi, Javad and Kar, Soummya},
  journal={IEEE Access},
  volume={7},
  pages={157535--157554},
  year={2019},
  publisher={IEEE}
}


@inproceedings{haddadpour2019trading,
  title={Trading Redundancy for Communication: Speeding up Distributed SGD for Non-convex Optimization},
  author={Haddadpour, Farzin and Kamani, Mohammad Mahdi and Mahdavi, Mehrdad and Cadambe, Viveck},
  booktitle={International Conference on Machine Learning},
  pages={2545--2554},
  year={2019}
}
@misc{FederatedAveragingAlgorithmn,
    author    = "Basil Han",
    title     = "Federated Averaging Algorithmn",
    url       = "https://medium.com/datadriveninvestor/an-overview-of-federated-learning-8a1a62b0600d"
}

@misc{Nist,
    author    = "National Institute of Standards and Technology",
    title     = "Emnist Dataset",
    url       = "https://www.nist.gov/srd/nist-special-database-19"
}
@misc{FederatedLearning1,
    author    = "TensorFlow Authors",
    title     = "Federated Learning for Image Classification", 
    url       = ""
}
